Dynamics Learning with Cascaded Variational Inference for Multi-Step Manipulation

The fundamental challenge of planning for multi-step manipulation is to find effective and plausible action sequences that lead to the task goal. We present Cascaded Variational Inference (CAVIN) Planner, a model-based method that hierarchically generates plans by sampling from latent spaces. To facilitate planning over long time horizons, our method learns latent representations that decouple the prediction of high-level effects from the generation of low-level motions through cascaded variational inference. This enables us to model dynamics at two different levels of temporal resolutions for hierarchical planning. We evaluate our approach in three multi-step robotic manipulation tasks in cluttered tabletop environments given high-dimensional observations. Empirical results demonstrate that the proposed method outperforms state-of-the-art model-based methods by strategically interacting with multiple objects.

==> deprecated-0-preamble.tex <==
% Author: Animesh Garg
% Date : July 2015
% This is a list of common packages needed in a wide range of latex docs for everyday writing.
% ---------------------------------
%floats and figures
% ---------------------------------
\usepackage{graphics}
\usepackage[pdftex]{graphicx}
\usepackage{wrapfig}
\DeclareGraphicsExtensions{.pdf,.png,.jpg}
%\pdfimageresolution200
\usepackage{epsfig}
\usepackage[font={small}]{caption}
\usepackage{subcaption}
%DONT USE BOTH SUBCAPTION AND SUBFIGURE
%\usepackage[center]{subfigure} 
% \usepackage{overpic}
\usepackage[rightcaption]{sidecap}
\usepackage{pbox}

\usepackage{bigstrut}
\setlength\bigstrutjot{3pt}

% ---------------------------------
%Math Stuff
% ---------------------------------
% Comments by Kuan: Below lines make some math notations misaligned or being bold in a weird way.

% \usepackage{mathtools}
% \usepackage{amsmath, amssymb, amscd}
% \usepackage{ wasysym } %special symbols
% \usepackage{amsfonts}
% \usepackage{mathptmx} % selects Times Roman as basic font
% \usepackage{gensymb} 
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% % \usepackage{mdwmath}
% % \usepackage{mdwtab}
% % \usepackage{eqparbox} %equations
% % \usepackage{mathtools}
% \numberwithin{equation}{section} 

% ---------------------------------
%Symbols
% ---------------------------------
\DeclareMathAlphabet{\mathcal}{OMS}{lmsy}{m}{n}
\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
\usepackage{textcomp} %for getting text tilde
%\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
%\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
%\usepackage{dsfont}

% ---------------------------------
%  Algorithms
% ---------------------------------
% http://tex.stackexchange.com/questions/229355/algorithm-algorithmic-algorithmicx-algorithm2e-algpseudocode-confused

\usepackage{algorithm} %float wrapper for algorithms. %dont use with algorithm2e
%should only use one of algorithmic or algorithmicx or algorithm2e
% \usepackage{algorithmic} %least preferred
% \usepackage[ruled,vlined,linesnumbered]{algorithm2e} 
\usepackage{algorithmicx, algpseudocode} %algpseudocode:layout for algorithmicx

% \algtext*{EndFunction}% Remove "end while" text
% \algtext*{EndWhile}% Remove "end while" text
% \algtext*{EndIf}% Remove "end if" text


% ---------------------------------
%Table Stuff
% ---------------------------------
\usepackage{array} %for table entries to be in center of cell
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}
\usepackage{tabulary}

% ---------------------------------
%DOCUMENT WIDE
% ---------------------------------
\usepackage[T1]{fontenc} 
    \usepackage{ae} %
    \usepackage{aecompl}
\usepackage[utf8]{inputenc}
\usepackage[protrusion=true,expansion=true]{microtype}
\usepackage[english]{babel} %for hyphenation rules
\usepackage{units}
\usepackage{siunitx}
\usepackage{bm}
\usepackage{times} % assumes new font selection scheme installed
\usepackage{xspace}
\usepackage{flushend}%balance columns on last page
\usepackage{balance} 
\usepackage{csquotes}
\usepackage{makeidx}
\usepackage{blindtext}

\let\labelindent\relax
\usepackage{enumitem}

\usepackage{tikz}
\usetikzlibrary{backgrounds}

\usepackage{ragged2e}
% \usepackage{fixltx2e} %fix latex issue across versions not needed in new latex versions
\usepackage{soul} %text highlighting
\usepackage{subfiles} %individual file compilation--makes it quick 

% \usepackage[protrusion=true,expansion=true]{microtype}
\setlength{\emergencystretch}{3em}

\usepackage[yyyymmdd]{datetime}
\renewcommand{\dateseparator}{-}
\date{\protect\formatdate{1}{1}{2001}}

% ---------------------------------
%Bibliography and cross-ref
% ---------------------------------
% The following lines are for IEEE style conflicts with natbibs
% \makeatletter
% \let\NAT@parse\undefined
% \makeatother
% \usepackage[numbers]{natbib}
% \usepackage{cite} %DONT USE NATBIB AND CITE TOGETHER

%hyperlinking
% \usepackage{url}
\makeatletter
% \g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother
\usepackage{color}
% \usepackage[usenames,dvipsnames,table]{xcolor}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}

% \usepackage{hyperref}
% \hypersetup{
%     colorlinks=true,
%     linkcolor=black,
%     citecolor=black,
%     filecolor=cyan,
%     urlcolor=black
% }

%=======U S E R  D E F I N E D  M A C R O S=======
% ---------------------------------
% User Comments
% ---------------------------------
\usepackage{marginnote}
% \newcommand{\bibhref}[2]{#2}
\usepackage{soul} %text highlighting
\newcommand{\todohl}[1]{{[\hl{#1?}]}}

%\usepackage[disable]{todonotes}
\usepackage[colorinlistoftodos,prependcaption,textsize=small]{todonotes}
\usepackage{regexpatch}
%\tracingxpatches%for debugging
\makeatletter
\xpatchcmd{\@todo}{\setkeys{todonotes}{#1}}{\setkeys{todonotes}{inline,#1}}{}{}
\makeatother

%takes in optional argument
\newcommand{\tocite}[1]{%
\textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}%
}

% \newcommand\todo[1]{{\color{red} TODO: #1 }}
\newcommand{\ignore}[1]{}
\newcommand{\etal}{et al.~}

%version in control in draft mode
\newcommand{\versionString}{\textcolor{red}{draft-mode-[\today\ \currenttime]}}

% ---------------------------------
% Label utils
% ---------------------------------

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure\,\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}


% ---------------------------------
% External refs
% ---------------------------------
\usepackage{xr}
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother
 
\newcommand*{\inputexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% space tweaks 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \setlength{\abovecaptionskip}{1mm}        
% \setlength{\belowcaptionskip}{1mm}        
% \setlength{\textfloatsep}{0mm}
% \setlength{\dbltextfloatsep}{3mm}
\renewcommand{\baselinestretch}{1.0}

\makeatletter
\newenvironment{mcases}[1][l]
 {\let\@ifnextchar\new@ifnextchar
  \left\lbrace
  \def\arraystretch{1.2}%
  \array{@{}l@{\quad}#1@{}}}
 {\endarray\right.}
\makeatother

==> depricated-1-intro-v2.tex <==
\vspace{-3pt}
\section{Introduction}
\vspace{-3pt}

Manipulation planning concerns the automatic generation of plans, \ie~sequences of actions, to change the states of movable objects for achieving a specified task goal. Consider tasks such as tool use~\cite{Toussaint2018DifferentiablePA} and manipulating among movable obstacles~\cite{Stilman2007ManipulationPA}, the agent needs to compose diverse actions into potential plans and choose the one best serves the purpose. As a result, the planned sequence of actions should not only effectively solves the puzzle step by step, but also produces a trajectory that is feasible under physical and semantic constraints of the environment. While planning in symbolic domains and known environments have been widely studied in the past, manipulation planning in the real world is substantially more challenging due to raw sensory inputs, unknown dynamics, high-dimensional state and action spaces, and long task horizons.


% Long-term robot autonomy in real-world environments involves reasoning and planning for multi-stage tasks. Consider problems such as task-oriented tool use ~\cite{Toussaint2018DifferentiablePA} and manipulation among movable objects~\cite{Stilman2007ManipulationPA}. Such tasks require an agent to plan for diverse interactions with different objects in the environment in order to reach the goal of the task. While planning in simple symbolic domains and known environments have been widely studied in the past, multi-stage robotic manipulation tasks in the real world are substantially more challenging due to raw sensory inputs, high-dimensional continuous action space and long task horizons.

To solve multiple tasks in unknown environments in a data-efficient manner, model-based approaches have been proposed to use learned dynamics models for planning~\cite{guo2014deep, Agrawal2016LearningTP, Finn2017DeepVF}. Given the trajectories predicted by the dynamics model, a plan can be selected by sampling-based planning algorithms~\cite{rubinstein2013cross}. These methods have shown successes in many control tasks given visual input data, such as playing video games~\cite{guo2014deep}, pushing a specified object in a cluttered tray~\cite{Finn2017DeepVF}, and manipulating deformable objects~\cite{nair2017combining}. However, directly planning in the original state and action space could be computationally intractable in complex manipulation planning problems. When there are multiple constraints and movable objects presented in the scene, a random trajectory uniformly sampled from a large state and action spaces would unlikely to have meaningful effects for the task. And it often can be infeasible due to collisions or other task constraints. When the task complexity is beyond what greedy strategies can solve, the difficulty of selecting an optimal plan is daunting with the dimensions of the state and action spaces and grows exponentially with respect to the task horizon. 

% where the order of the interacted objects is not specified and multiple constraints are presented, a random action uniformly sampled from the high-dimensional action space is most likely to be effective or infeasible. As a result, planning in the original state and action space will be not sample-efficient. 

% We address the problem of planning for multi-stage tasks with a model-based approach. At the heart of model-based methods is a dynamics model and a sample distribution. that predicts the effects of actions to the environment. Given a dynamics model, the \emph{plan}, \ie~a sequence of actions, can be produced by sampling-based and gradient-based planning algorithms~\cite{rubinstein2013cross, srinivas2018universal}. While perfectly modeling the environment is usually infeasible, the recent advances in deep learning have inspired a number of approaches to predict dynamics in either observation spaces~\cite{Finn2017DeepVF, Ebert2018VisualFM} or latent spaces~\cite{Watter2015EmbedTC, Agrawal2016LearningTP, srinivas2018universal, Hafner2018LearningLD, janner2019reasoning} through representation learning. These methods have shown successes in a wide range of continuous control tasks given raw sensory observations received from the environment.

% We address the problem of planning for multi-stage tasks with a model-based reinforcement learning (RL)~\cite{sutton2018reinforcement} approach. At the heart of model-based methods is a \emph{dynamics model} that predicts the effects of actions to the environment. Given a dynamics model, the \emph{plan}, \ie~a sequence of actions, can be produced by sampling-based and gradient-based planning algorithms~\cite{rubinstein2013cross, srinivas2018universal}. While perfectly modeling the environment is usually infeasible, the recent advances in deep learning have inspired a number of approaches to predict dynamics in either observation spaces~\cite{Finn2017DeepVF, Ebert2018VisualFM} or latent spaces~\cite{Watter2015EmbedTC, Agrawal2016LearningTP, srinivas2018universal, Hafner2018LearningLD, janner2019reasoning} through representation learning. These methods have shown successes in a wide range of continuous control tasks given raw sensory observations received from the environment.

% In this work, we want to\todo{say the characteristics of our task that make it hard} 

% However, directly applying existing model-based methods to tasks of higher complexities could be ineffective. These methods are faced with two major limitations: First, learning an accurate and generalizable dynamicsan model which can accurately predict outcomes of arbitrary actions would require huge amount of data and enormous model capacity. Second, even with a perfectly trained dynamics model, finding the optimal plan for a complex task could be computationally impracticable, as the complexity of action selection is daunting with high-dimensional continuous action space and grows exponentially with respect to the task horizon. 

% \todo{In this paragraph state clearly what kinds of abstraction people have investigated, what is our abstraction (action abstraction), what people have tried for action abstraction, and then introduce "action mode" and say why it's different and better than prior approaches}
 
This problem is oft-studied with two major lines of attack.  The first one is planning with abstract symbolic states~\cite{kaelbling2011hierarchical}. Albeit, combining it with continuous decisions results in combinatorial problem size. A recent line of inquiry explores amalgamation of discrete logic programming with differentiable physics model~\cite{Toussaint2018DifferentiablePA}. However, it requires a known, simplified dynamics model operating on privileged state information. 
%RL does not scale to multi-stage tasks
Second approach is data-driven learning. Model-free reinforcement learning (RL) has pushed the boundaries enabling domain-independent visual input and complicated dynamics~\cite{kalashnikov2018qt}. Albeit, these methods do not extend to multi-stage manipulation in part because of non-intuitive multi-step reward function specification, the need for structured exploration, and poor sample efficiency of Deep RL methods.
In contrast, Model-based RL (MBRL) methods have shown promise in face of these challenges. MBRL methods fit a dynamics model (often in high-dimensional state space) and thereafter leverage it for planning, either through optimization~\cite{Watter2015EmbedTC} or through sampling~\cite{guo2014deep, Agrawal2016LearningTP, Finn2017DeepVF}. However, dynamics learning techniques herein limited by the myopic prediction accuracy, inability to capture multi-modality, and lack of multi-resolution prediction --- thereby precluding their use in closed-loop, task-aware, long-horizon planning. 

% this paper
% Further multi-resolution reasoning is not exhibited and hence greedy only decision making can be done -- switching contacts in a single planning episode requires a task-awareness.
% The main challenge is to build multi-resolution dynamics models that can be guide task-aware discrete decisions as well as continuous motions. 

We introduce the \algoFull (\algoName) model to enable hierarchical planning in multi-stage tasks. The main insight is that we can sample actions in a two-stage cascade process: a high-level plan of desired effects predicted at a coarse temporal resolution, and a low-level plan of motion at a fine-grained resolution. Through the decoupling of effect and motion, we effectively reduce the search space of the optimal plan, enabling \algoName to solve longer-horizon manipulation tasks with high-dimensional states and continuous actions.


% that a factorized dynamics model with factorized action spaces, which enables goal-driven, long-term planning while balancing short-term motion-scale feasibility. Planning in a fine-grained temporal resolution yields a computationally challenging problem, especially with high-dimensional states and continuous actions. In contrast we decompose the planning into a , where the search space of the optimal plan can be efficiently reduced. Our model first produces a high-level 
% Hence, we build on two ideas: (a) an “intuitive physics engine” can forward simulate the outcome of an action in latent perceptual space, and (b) it should be factorized to sample both long-term and short-term actions.
% The \textit{latent intention} is first selected to decide a plan sketch as a achievable sequence of states that can lead to the task goal, regardless of the motion trajectories of the actions. Then the \textit{latent motion} is planned to generate a feasible sequence of actions according to the plan sketch for the robot to execute. 


Our contributions of this work are three-fold:

\noindent
1. We introduce \algoName, which exploits the hierarchical factorization of dynamics for model-based planning. It decouples the high-level prediction of effects from the low-level generation of motions. We use conditional generative models to learn dynamics models at two levels of temporal resolutions. We employ variational principles~\cite{kingma2013auto} to derive lower bound objectives for training the model.

\noindent
2. We introduce a cascade process to effectively sample actions with \algoName. We perform model predictive control (MPC) at the two temporal resolutions to generate plans. %The high-level plans indicate the desired effects on the objects in order to complete a task. The corresponding low-level plans determine the fine-grained actions to realize these desired effects. 
Such temporal abstraction substantially reduces the computational burden of sampling long sequences of continuous actions.

% 2. The latent representations and the cascaded generative model are jointly learned through variational inference. To encourage learning structures in the latent representation, we add an \textit{intention consistency loss} during training, in order to ensure that the motion trajectory is consistent with the plan sketch. Combining this loss with the evidence lower bound~\cite{kingma2013auto} yields the full objective of the learning, which results in informative and effective latent spaces for planning.

\noindent
3. We demonstrate the effectiveness of the proposed model in three multi-stage manipulation tasks. These tasks are designed to highlight different challenges: task constraints (\texttt{Insertion}), motion constraints (\texttt{Crossing}), and multi-object interactions (\texttt{Clearing}). Our factorized dynamics model (\algoName) outperforms several strong model-based baselines on all three tasks.

Additional details at \href{https://sites.google.com/view/cavin}{\small \texttt{sites.google.com/view/cavin}}.


% These tasks involve an articulated arm interacting with multiple objects in a cluttered environment for achieving predefined task goals. We compare the proposed approach the model predictive controllers without using the actions modes. 
% Empirical results demonstrate that using the S-MPC model boost the performance of the three tasks.  


% First, we can train models of sensory observations, i.e. video prediction models, from completely unlabeled interaction data requiring no manual annotation. Second, low-level sensory observations such as pixels include all information about the environment that the robot can currently perceive, and hence are general to a wide range of objects and situations, including nonrigid and deformable objects. 



% Building realistic models of multi-object, nonprehensile interactions is challenging with analytic methods, as friction and contact dynamics become extraordinarily complex [15], and inferring them directly from images is

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/pull-fig.png}
    \caption{(a) Multi-Stage Crossing Task: move target object to goal along the path. A potential 3-step high-level plan is illustrated. (b) In presence of an obstacle, the planner needs move the obstacle aside and then move the target. (c) This reactive multi-resolution planning behavior is achieved through a hierarchical dynamics model (\algoName) that reasons over multiple temporal resolutions. \algoName samples context dependent sequence of high-level effect codes, which in turn guides motion and action sampling at the low-level to achieve task- completion in continuous state-action space without explicit symbolic planning.}
    \label{fig:main}
    \vspace{-15pt}
\end{figure*}

==> latexmkrc <==
#custom changes to refer appendix in main doc
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );
 
        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );
 
        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
 
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
